Whole-Body Control of a Mobile Manipulator using End-to-End Reinforcement Learning

Mobile manipulation is usually achieved by sequentially executing base and manipulator movements. This simplification, however, leads to a loss in efficiency and in some cases a reduction of workspace size. Even though different methods have been proposed to solve Whole-Body Control (WBC) online, they are either limited by a kinematic model or do not allow for reactive, online obstacle avoidance. In order to overcome these drawbacks, in this work, we propose an end-to-end Reinforcement Learning (RL) approach to WBC. We compared our learned controller against a state-of-the-art sampling-based method in simulation and achieved faster overall mission times. In addition, we validated the learned policy on our mobile manipulator RoyalPanda in challenging narrow corridor environments.

==> acronyms.tex <==
\acro{rl}{RL}{Reinforcement Learning}
\newacronym{mpc}{MPC}{Model Predictive Control}
\newacronym{nmpc}{NMPC}{Nonlinear Model Predictive Control}
\newacronym{dmpc}{DMPC}{Deep Value Model Predictive Control}
\newacronym{mav}{MAV}{Micro Aerial Vehicle}
\newacronym{slq}{SLQ}{Sequential Linear Quadratic}
\newacronym{ram}{RAM}{Random Access Memory}
\newacronym{wbc}{WBC}{Whole Body Control}
\newacronym{ros}{ROS}{Robot Operating System}
\newacronym{slam}{SLAM}{Simultaneous Localization and Mapping}
\newacronym{tsdf}{TSDF}{Truncated Signed Distance Field}
\newacronym{rms}{RMS}{Root Mean Square}
\newacronym{mdp}{MDP}{Markov Decision Process}
\newacronym{arc}{ARC}{Amazon Robotics Challenge}
\newacronym{dof}{DoF}{Degrees of Freedom}
\newacronym{ppo}{PPO}{Proximal Policy Optimization}
\newacronym{ddpg}{DDPG}{Deep Deterministic Policy Gradient}
\newacronym{trpo}{TRPO}{Trust Region Policy Optimization}
\newacronym{ac}{AC}{Actor-Critic}
\newacronym{mlp}{MLP}{Multi-layer perceptron}
\newacronym{rnn}{RNN}{Recurrent Neural Network}
\newacronym{adr}{ADR}{Automatic Domain Randomization}
\newacronym{hpt}{HPT}{Harmonic Potential Field}
\newacronym{lidar}{LiDAR}{Light Detection And Ranging}

==> pgfplots_preamble.tex <==
\makeatletter

\newif\ifpgfplots@scaled@x@ticks@engineering
\pgfplots@scaled@x@ticks@engineeringfalse
\newif\ifpgfplots@scaled@y@ticks@engineering
\pgfplots@scaled@y@ticks@engineeringfalse
\newif\ifpgfplots@scaled@z@ticks@engineering
\pgfplots@scaled@z@ticks@engineeringfalse

\pgfplotsset{
    scaled x ticks/engineering/.code=
        \pgfplots@scaled@x@ticks@engineeringtrue,
    scaled y ticks/engineering/.code=
        \pgfplots@scaled@y@ticks@engineeringtrue,
    scaled z ticks/engineering/.code=
        \pgfplots@scaled@y@ticks@engineeringtrue,
%    scaled ticks=engineering  % Uncomment this line if you want "engineering" to be on by default
}

\def\pgfplots@init@scaled@tick@for#1{%
    \global\def\pgfplots@glob@TMPa{0}%
    \expandafter\pgfplotslistcheckempty\csname pgfplots@prepared@tick@positions@major@#1\endcsname
    \ifpgfplotslistempty
        % we have no tick labels. Omit the tick scale label as well!
    \else
    \begingroup
    \ifcase\csname pgfplots@scaled@ticks@#1@choice\endcsname\relax
    % CASE 0 : scaled #1 ticks=false: do nothing here.
    \or
        % CASE 1 : scaled #1 ticks=true:
        %--------------------------------
        % the \pgfplots@xmin@unscaled@as@float  is set just before the data
        % scale transformation is initialised.
        %
        % The variables are empty if there is no datascale transformation.
        \expandafter\let\expandafter\pgfplots@cur@min@unscaled\csname pgfplots@#1min@unscaled@as@float\endcsname
        \expandafter\let\expandafter\pgfplots@cur@max@unscaled\csname pgfplots@#1max@unscaled@as@float\endcsname
        %
        \ifx\pgfplots@cur@min@unscaled\pgfutil@empty
            \edef\pgfplots@loc@TMPa{\csname pgfplots@#1min\endcsname}%
            \expandafter\pgfmathfloatparsenumber\expandafter{\pgfplots@loc@TMPa}%
            \let\pgfplots@cur@min@unscaled=\pgfmathresult
            \edef\pgfplots@loc@TMPa{\csname pgfplots@#1max\endcsname}%
            \expandafter\pgfmathfloatparsenumber\expandafter{\pgfplots@loc@TMPa}%
            \let\pgfplots@cur@max@unscaled=\pgfmathresult
        \fi
        %
        \expandafter\pgfmathfloat@decompose@E\pgfplots@cur@min@unscaled\relax\pgfmathfloat@a@E
        \expandafter\pgfmathfloat@decompose@E\pgfplots@cur@max@unscaled\relax\pgfmathfloat@b@E
        \pgfplots@init@scaled@tick@normalize@exponents
        \ifnum\pgfmathfloat@b@E<\pgfmathfloat@a@E
            \pgfmathfloat@b@E=\pgfmathfloat@a@E
        \fi
        \xdef\pgfplots@glob@TMPa{\pgfplots@scale@ticks@above@exponent}%
        \ifnum\pgfplots@glob@TMPa<\pgfmathfloat@b@E
            % ok, scale it:
            \expandafter\ifx % Check whether we're using engineering notation (restricting exponents to multiples of three)
                \csname ifpgfplots@scaled@#1@ticks@engineering\expandafter\endcsname
                \csname iftrue\endcsname
                    \divide\pgfmathfloat@b@E by 3
                    \multiply\pgfmathfloat@b@E by 3
            \fi
            \multiply\pgfmathfloat@b@E by-1
            \xdef\pgfplots@glob@TMPa{\the\pgfmathfloat@b@E}%
        \else
            \xdef\pgfplots@glob@TMPa{\pgfplots@scale@ticks@below@exponent}%
            \ifnum\pgfplots@glob@TMPa>\pgfmathfloat@b@E
                % ok, scale it:
                \expandafter\ifx % Check whether we're using engineering notation (restricting exponents to multiples of three)
                    \csname ifpgfplots@scaled@#1@ticks@engineering\expandafter\endcsname
                    \csname iftrue\endcsname
                        \advance\pgfmathfloat@b@E by -2
                        \divide\pgfmathfloat@b@E by 3
                        \multiply\pgfmathfloat@b@E by 3
                \fi
                \multiply\pgfmathfloat@b@E by-1
                \xdef\pgfplots@glob@TMPa{\the\pgfmathfloat@b@E}%
            \else
                % no scaling necessary:
                \xdef\pgfplots@glob@TMPa{0}%
            \fi
        \fi
    \or
        % CASE 2 : scaled #1 ticks=base 10:
        %--------------------------------
        \c@pgf@counta=\csname pgfplots@scaled@ticks@#1@arg\endcsname\relax
        %\multiply\c@pgf@counta by-1
        \xdef\pgfplots@glob@TMPa{\the\c@pgf@counta}%
    \or
        % CASE 3 : scaled #1 ticks=real:
        %--------------------------------
        \pgfmathfloatparsenumber{\csname pgfplots@scaled@ticks@#1@arg\endcsname}%
        \global\let\pgfplots@glob@TMPa=\pgfmathresult
    \or
        % CASE 4 : scaled #1 ticks=manual:
        \expandafter\global\expandafter\let\expandafter\pgfplots@glob@TMPa\csname pgfplots@scaled@ticks@#1@arg\endcsname
    \fi
    \endgroup
    \fi
    \expandafter\let\csname pgfplots@tick@scale@#1\endcsname=\pgfplots@glob@TMPa%
}
\makeatother
